The network survival method for estimating adult mortality: Evidence from a survey experiment in Rwanda

Adult death rates are a critical indicator of population health and wellbeing. Wealthy countries have high-quality vital registration systems, but poor countries lack this infrastructure and must rely on estimates that are often problematic. In this paper, we introduce the network survival method, a new approach for estimating adult death rates. We derive the precise conditions under which it produces estimates that are consistent and unbiased. Further, we develop an analytical framework for sensitivity analysis. To assess the performance of the network survival method in a realistic setting, we conducted a nationally-representative survey experiment in Rwanda (n=4,669). Network survival estimates were similar to estimates from other methods, even though the network survival estimates were made with substantially smaller samples and are based entirely on data from Rwanda, with no need for model life tables or pooling of data from other countries. Our analytic results demonstrate that the network survival method has attractive properties, and our empirical results show that it can be used in countries where reliable estimates of adult death rates are sorely needed.

==> figures/from_code/ffqf-table.tex <==

% Table created by stargazer v.5.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Sat, Feb 18, 2017 - 09:14:54 PM
\begin{table}[!htbp] \centering 
  \caption{Estimated $\ffqf$ values, by tie definition and sex, along with summaries of
the estimated sampling distribution for each estimator. The coefficient of variation is
the estimated standard error divided by the estimated mean; it is comparable across the
different estimates.} 
  \label{tab:ffqf} 
\small 
\begin{tabular}{@{\extracolsep{5pt}} ccccccc} 
\\[-1.8ex]\hline \\[-1.8ex] 
Tie definition & Sex & mean & median & std. error & coef. of variation & 95\% CI \\ 
\hline \\[-1.8ex] 
Acquaintance & female & $0.19$ & $0.18$ & $0.02$ & $0.11$ & [0.15-0.23] \\ 
Meal & female & $0.24$ & $0.24$ & $0.03$ & $0.12$ & [0.19-0.30] \\ 
Sibling & female & $0.17$ & $0.17$ & $0.01$ & $0.08$ & [0.15-0.20] \\ 
Acquaintance & male & $0.26$ & $0.26$ & $0.02$ & $0.09$ & [0.22-0.31] \\ 
Meal & male & $0.26$ & $0.26$ & $0.03$ & $0.10$ & [0.21-0.32] \\ 
Sibling & male & $0.28$ & $0.28$ & $0.02$ & $0.08$ & [0.23-0.32] \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> figures/from_code/num-deaths-allage-overdisp.tex <==

% Table created by stargazer v.5.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Sat, Feb 18, 2017 - 09:05:06 PM
\begin{table}[!htbp] \centering 
  \caption{Average, Variance, Average/Variance, and Maximum of the number of deaths of all ages reported by respondents to the network reporting survey, by tie definition. The ratio (Average / Variance) in the number of reported deaths would be expected to be 1 if the responses followed a Poisson distribution; higher values suggest that there is overdispersion relative to a Poisson distribution.} 
  \label{tab:numdeathsoverdispallage} 
\small 
\begin{tabular}{@{\extracolsep{5pt}} ccccc} 
\\[-1.8ex]\hline \\[-1.8ex] 
Tie definition & Avg. Num. Reported deaths & Var. in Num. Reported Deaths & (Avg. / Var.) in Num. Reported Deaths & Max. Num. Reported Deaths \\ 
\hline \\[-1.8ex] 
Acquaintance & $1.13$ & $1.95$ & $1.73$ & $12$ \\ 
Meal & $0.54$ & $1.09$ & $2.04$ & $10$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> figures/from_code/num-deaths-overdisp-all.tex <==

% Table created by stargazer v.5.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Sat, Feb 18, 2017 - 09:05:07 PM
\begin{table}[!htbp] \centering 
  \caption{Average, Variance, Average/Variance, and Maximum of the number of adult deaths (ages 15-64) reported by respondents to the network reporting survey, by tie definition. The ratio (Average / Variance) in the number of reported deaths would be expected to be 1 if the responses followed a Poisson distribution; higher values suggest that there is overdispersion relative to a Poisson distribution.} 
  \label{tab:allnumdeathsoverdisp} 
\small 
\begin{tabular}{@{\extracolsep{5pt}} ccccc} 
\\[-1.8ex]\hline \\[-1.8ex] 
Tie definition & Avg. Num. Reported deaths & Var. in Num. Reported Deaths & (Avg. / Var.) in Num. Reported Deaths & Max. Num. Reported Deaths \\ 
\hline \\[-1.8ex] 
Acquaintance & $0.74$ & $1.17$ & $1.58$ & $10$ \\ 
Meal & $0.39$ & $0.69$ & $1.78$ & $9$ \\ 
Sibling (12 months) & $0.01$ & $0.01$ & $1.07$ & $3$ \\ 
Sibling (84 months) & $0.09$ & $0.11$ & $1.23$ & $4$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> figures/from_code/num-deaths-overdisp.tex <==

% Table created by stargazer v.5.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Sat, Feb 18, 2017 - 09:05:06 PM
\begin{table}[!htbp] \centering 
  \caption{Average, Variance, Average/Variance, and Maximum of the number of deaths in ages 15-65 reported by respondents to the network reporting survey, by tie definition. The ratio (Average / Variance) in the number of reported deaths would have expected value 1 if the responses followed a Poisson distribution; higher values suggest that there is overdispersion relative to a Poisson distribution.} 
  \label{tab:numdeathsoverdisp} 
\small 
\begin{tabular}{@{\extracolsep{5pt}} ccccc} 
\\[-1.8ex]\hline \\[-1.8ex] 
Tie definition & Avg. Num. Reported deaths & Var. in Num. Reported Deaths & (Avg. / Var.) in Num. Reported Deaths & Max. Num. Reported Deaths \\ 
\hline \\[-1.8ex] 
Acquaintance & $0.74$ & $1.17$ & $1.58$ & $10$ \\ 
Meal & $0.39$ & $0.69$ & $1.78$ & $9$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> figures/from_code/num-deaths-rep-byover50.tex <==

% Table created by stargazer v.5.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Sat, Feb 18, 2017 - 09:05:07 PM
\begin{table}[!htbp] \centering 
  \caption{Average number of reported deaths, by tie defintion, and by whether or not respondents are over age 50.} 
  \label{tab:deathrepbyage} 
\small 
\begin{tabular}{@{\extracolsep{5pt}} cccc} 
\\[-1.8ex]\hline \\[-1.8ex] 
Tie definition & Over 50 & Avg. Num. Reported Deaths & Num. Interviews \\ 
\hline \\[-1.8ex] 
Acquaintance & FALSE & $0.75$ & $1,896$ \\ 
Acquaintance & TRUE & $0.70$ & $363$ \\ 
Meal & FALSE & $0.39$ & $1,997$ \\ 
Meal & TRUE & $0.37$ & $407$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 

